Low Complexity Blind Equalization for OFDM Systems with General Constellations

This paper proposes a low-complexity algorithm for blind equalization of data in OFDM-based wireless systems with general constellations. The proposed algorithm is able to recover data even when the channel changes on a symbol-by-symbol basis, making it suitable for fast fading channels. The proposed algorithm does not require any statistical information of the channel and thus does not suffer from latency normally associated with blind methods. We also demonstrate how to reduce the complexity of the algorithm, which becomes especially low at high SNR. Specifically, we show that in the high SNR regime, the number of operations is of the order O(LN), where L is the cyclic prefix length and N is the total number of subcarriers. Simulation results confirm the favorable performance of our algorithm.

==> new_commands.tex <==
\newcommand{\x}{\mbox{\boldmath $x$}}
\newcommand{\n}{\mbox{\boldmath $n$}}
\newcommand{\sh}{\mbox{\boldmath $\underline{h}$}}
\newcommand{\she}{\mbox{\boldmath ${h}$}}
\newcommand{\uu}{\mbox{\boldmath $\underline{x}$}}
\newcommand{\vzero}{\mbox{\boldmath $0$}}
\newcommand{\y}{\mbox{\boldmath $y$}}
\newcommand{\X}{\mbox{${\mathcal X}$}}
\newcommand{\xx}{\mbox{${\mathcal x}$}}
\newcommand{\calH}{\mbox{\boldmath ${\mathcal H}$}}
\newcommand{\calX}{\mbox{\boldmath ${\mathcal X}$}}
\newcommand{\calY}{\mbox{\boldmath ${\mathcal Y}$}}
\newcommand{\calN}{\mbox{\boldmath ${\mathcal N}$}}
\newcommand{\calD}{\mbox{\boldmath ${\mathcal D}$}}
\newcommand{\z}{\mbox{\boldmath $\underline{z}$}}
\newcommand{\mh}{\mbox{\boldmath $H$}}
\newcommand{\deltau}{\mbox{\boldmath $\underline{\delta x}$}}
\newcommand{\deltaB}{\mbox{\boldmath $\delta $}}
\newcommand{\w}{\mbox{\boldmath $w$}}
\newcommand{\wo}{\mbox{\boldmath $w_{o}$}}
\newcommand{\qq}{\mbox{\boldmath $q$}}
\newcommand{\J}{\mbox{\boldmath $J$}}
\newcommand{\II}{\mbox{\boldmath $I$}}
\newcommand{\AC}{\mbox{\boldmath $R$}}
\newcommand{\veczero}{\mbox{\boldmath{$0$}}}
\newcommand{\QQ}{\mbox{\boldmath $Q$}}
\newcommand{\BQ}{\mbox{\boldmath $Q$}}
\newcommand{\BC}{\mbox{\boldmath $C$}}
\newcommand{\BD}{\mbox{\boldmath $D$}}
\newcommand{\W}{\mbox{\boldmath $W$}}
\newcommand{\C}{\mbox{\boldmath $C$}}
\newcommand{\A}{\mbox{\boldmath $A$}}
\newcommand{\BA}{\mbox{\boldmath $A$}}
\newcommand{\BF}{\mbox{\boldmath $F$}}
\newcommand{\BG}{\mbox{\boldmath $G$}}
\newcommand{\BB}{\mbox{\boldmath $B$}}
\newcommand{\BPi}{\mbox{\boldmath $\Pi$}}
\newcommand{\BP}{\mbox{\boldmath $P$}}
\newcommand{\BK}{\mbox{\boldmath $K$}}
\newcommand{\BR}{\mbox{\boldmath $R$}}
\newcommand{\BPhi}{\mbox{\boldmath $\Phi$}}
\newcommand{\Bb}{\mbox{\boldmath $b$}}
\newcommand{\Bu}{\mbox{\boldmath $u$}}
\newcommand{\Btheta}{\mbox{\boldmath $\theta$}}
\newcommand{\OO}{\mbox{\boldmath $O$}}
\newcommand{\Bq}{\mbox{\boldmath $q$}}
\newcommand{\bigO}{\mbox{\boldmath $\large O$}}
\newcommand{\BX}{\mbox{\boldmath $X$}}
\newcommand{\BW}{\mbox{\boldmath $W$}}
\newcommand{\BH}{\mbox{\boldmath $H$}}
\newcommand{\BI}{\mbox{\boldmath $I$}}
\newcommand{\BDelta}{\mbox{\boldmath $\Delta$}}
\newcommand{\Bw}{\mbox{\boldmath $w$}}
\newcommand{\Bk}{\mbox{\boldmath $k$}}
\newcommand{\Bh}{\mbox{\boldmath $h$}}
\newcommand{\Bm}{\mbox{\boldmath $m$}}
\newcommand{\BM}{\mbox{\boldmath $M$}}
\newcommand{\Bc}{\mbox{\boldmath $c$}}
\newcommand{\Ba}{\mbox{\boldmath $a$}}
\newcommand{\Br}{\mbox{\boldmath $r$}}
\newcommand{\ff}{\mbox{\boldmath $f$}}


\newcommand{\bq}{\begin{eqnarray}}
\newcommand{\eq}{\end{eqnarray}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeq}{\end{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\bqn}{\begin{eqnarray*}}
\newcommand{\eqn}{\end{eqnarray*}}
\newcommand{\ba}{\left[ \begin{array}}
\newcommand{\ea}{\\ \end{array} \right]}


\newcommand{\vv}{\mbox{\boldmath $w$}}
\newcommand{\B}{\mbox{\boldmath $B$}}
\newcommand{\PP}{\mbox{\boldmath $P$}}
\newcommand{\G}{\mbox{\boldmath $G$}}
\newcommand{\K}{\mbox{\boldmath $K$}}
\newcommand{\LL}{\mbox{\boldmath $L$}}
\newcommand{\define}{\stackrel{\Delta}{=}}
\newcommand{\M}{\mbox{\boldmath $M$}}
\newcommand{\Q}{\mbox{\boldmath $Q$}}

\newcommand{\si}{\mbox{$\Sigma$}}
\newcommand{\sib}{\mbox{$\overline{\sigma}$}}
\newcommand{\Si}{\mbox{\boldmath $\Sigma$}}
\newcommand{\Sib}{\mbox{\boldmath $\overline{\Sigma}$}}
\newcommand{\sla}{\mbox{\boldmath $\lambda$}}  %small bold lambda
\newcommand{\ssi}{\mbox{\boldmath $\sigma$}}  %small bold sigma
\newcommand{\ssib}{\mbox{\boldmath $\overline{\sigma}$}}  %small bold sigma
\newcommand{\la}{\mbox{$\Lambda$}}
\newcommand{\La}{\mbox{\boldmath $\Lambda$}}
\newcommand{\F}{\mbox{\boldmath $F$}}
\newcommand{\1}{\mbox{\boldmath $1$}}
\newcommand{\mus}{\mbox{$\overline{\mu}_{\Sigma}$}}
\newcommand{\eas}{\mbox{$e_a^{\Sigma}$}}
\newcommand{\eps}{\mbox{$e_p^{\Sigma}$}}
\newcommand{\wis}{\mbox{$\|\tilde{\w}_{i}\|$}}
\newcommand{\wips}{\mbox{$\|\tilde{\w}_{i+1}\|$}}
\newcommand{\wisb}{\mbox{$\|\overline{\w}_{i}\|$}}
\newcommand{\wipsb}{\mbox{$\|\overline{\w}_{i+1}\|$}}
\newcommand{\uisb}{\mbox{$\|\overline{\u}_{i}\|$}}
\newcommand{\uis}{\mbox{$\|\u_{i}\|$}}
\newcommand{\qis}{\mbox{$\|\qq_{i}\|$}}
\newcommand{\kr}{\mbox{$ \otimes $}}

\def\overu{\mbox{$\overline{\u}$}}
\def\over2u{\mbox{$\overline{\overline{\u}}$}}
\def\u{{\bf u}}

